EAIRA: Establishing a Methodology for Evaluating AI Models as Scientific Research Assistants

Recent advancements have positioned AI, and particularly Large Language Models (LLMs), as transformative tools for scientific research, capable of addressing complex tasks that require reasoning, problem-solving, and decision-making. Their exceptional capabilities suggest their potential as scientific research assistants but also highlight the need for holistic, rigorous, and domain-specific evaluation to assess effectiveness in real-world scientific applications. This paper describes a multifaceted methodology for Evaluating AI models as scientific Research Assistants (EAIRA) developed at Argonne National Laboratory. This methodology incorporates four primary classes of evaluations. 1) Multiple Choice Questions to assess factual recall; 2) Open Response to evaluate advanced reasoning and problem-solving skills; 3) Lab-Style Experiments involving detailed analysis of capabilities as research assistants in controlled environments; and 4) Field-Style Experiments to capture researcher-LLM interactions at scale in a wide range of scientific domains and applications. These complementary methods enable a comprehensive analysis of LLM strengths and weaknesses with respect to their scientific knowledge, reasoning abilities, and adaptability. Recognizing the rapid pace of LLM advancements, we designed the methodology to evolve and adapt so as to ensure its continued relevance and applicability. This paper describes the methodology state at the end of February 2025. Although developed within a subset of scientific domains, the methodology is designed to be generalizable to a wide range of scientific domains.

==> src/Related_ChemMat.tex <==
\subsubsection{Chemistry}
Numerous benchmarks have been developed to evaluate the capabilities of LLMs in chemistry and material science.
ChemistryQA \citep{wei_chemistryqa_2020}, an early question-answer dataset developed to evaluate language models, comprises 4500 complex questions that requires reasoning and calculations. 
\cite{white_assessment_2023} evaluated LLMs based on their code generation ability for 84 computational chemistry tasks and demonstrated 30\% increase in accuracy with prompt engineering. 
\cite{guo_what_2023} developed ChemLLMBenchmark, which is composed of eight practical chemistry tasks that requires understanding, reasoning, and explaining abilities. 
They evaluated five LLMs (GPT-4, GPT-3.5, Davinci-003, Llama, Galactica) using in-context learning and prompts designed for each task. 
Their study demonstrated the importance of in-context learning, as it improved the accuracy for all the tasks.
ChemBench \citep{mirza2024chembench} is an automated framework designed to be compatible with BigBench \citep{srivastava2023bigbench}.  ChemBench currently have more than 2700 questions, which are mainly generated semi-automatically or curated from different resources (textbooks, exams, lectures, etc). 
While the majority of the questions are MCQs, there are more than 240 open-ended questions as well.
MoleculeQA \citep{lu_moleculeqa_2024} is another question-answer dataset composed of 61,574 MCQs (three distractors for each question) for more than 23k molecules.
The questions are based on factual information (structural information, properties, application areas, and source of origin) about these molecules and are automatically generated based on templates.
The recently introduced MolPuzzle \citep{guo_can_2024} multimodal benchmark is based on deducing molecular structures from spectral data. 
The benchmark consists of more than 23k question-answer pairs with three interlinked sequential sub-tasks that evaluate molecule understanding, spectrum interpretation, and molecule
construction.
TOMG-Bench \citep{li_tomg-bench_2024} is an open-domain molecule generation benchmark composed of three  tasks: molecule edition, molecule optimization, and customized molecule generation. 
Each task has three subtasks comprised with 5000 samples, which are evaluated for both accuracy and quality. 
The evaluation metrics is specialized for the subtasks and can be automatically evaluated.
TOMG-Bench provides a leaderboard of 25 LLMs based on the weighted average of the accuracy scores.

